Harmful Terms and Where to Find Them: Measuring and Modeling Unfavorable Financial Terms and Conditions in Shopping Websites at Scale

Terms and conditions for online shopping websites often contain terms that can have significant financial consequences for customers. Despite their impact, there is currently no comprehensive understanding of the types and potential risks associated with unfavorable financial terms. Furthermore, there are no publicly available detection systems or datasets to systematically identify or mitigate these terms. In this paper, we take the first steps toward solving this problem with three key contributions. \textit{First}, we introduce \textit{TermMiner}, an automated data collection and topic modeling pipeline to understand the landscape of unfavorable financial terms. \textit{Second}, we create \textit{ShopTC-100K}, a dataset of terms and conditions from shopping websites in the Tranco top 100K list, comprising 1.8 million terms from 8,251 websites. Consequently, we develop a taxonomy of 22 types from 4 categories of unfavorable financial terms -- spanning purchase, post-purchase, account termination, and legal aspects. \textit{Third}, we build \textit{TermLens}, an automated detector that uses Large Language Models (LLMs) to identify unfavorable financial terms. Fine-tuned on an annotated dataset, \textit{TermLens} achieves an F1 score of 94.6\% and a false positive rate of 2.3\% using GPT-4o. When applied to shopping websites from the Tranco top 100K, we find that 42.06\% of these sites contain at least one unfavorable financial term, with such terms being more prevalent on less popular websites. Case studies further highlight the financial risks and customer dissatisfaction associated with unfavorable financial terms, as well as the limitations of existing ecosystem defenses.

==> fig_tex/finetune_stats.tex <==
\begin{figure}[!t] 
 \centering
 \includegraphics[width=0.45\textwidth,height=0.2\textheight]{imgs/placeholder.png}
 \caption{Model Performance versus size of fine-tuning data points.}
\label{fig:fintune}
\end{figure}

% [width=0.99\columnwidth]

==> fig_tex/rank_distribution.tex <==
\begin{figure}[!t] 
 \centering
 \includegraphics[width=0.99\columnwidth]{imgs/financial_terms_tranco.pdf}
 \caption{Number of websites with different categories of \termname terms in the Tranco top 80k websites. }
\label{fig:tranco_rank_dist}
\end{figure}


==> fig_tex/roc.tex <==
\begin{figure}[!t] 
 \centering
 \includegraphics[width=0.99\columnwidth]{imgs/roc_curve.pdf}
 \caption{Receiver Operating Characteristic (ROC) curve of different LLM's performance on the annotated dataset. }
\label{fig:roc}
\end{figure}


==> fig_tex/term_length_cdf.tex <==
\begin{figure}[!t] 
 \centering
 \includegraphics[width=0.95\columnwidth]{imgs/term_length_cdf.pdf}
 \caption{CDF of the length of terms in the T\&Cs across \websitecnt websites.}
\label{fig:term_length_cdf}
\end{figure}

==> fig_tex/user_star.tex <==
\begin{figure}[!t] 
 \centering
 \includegraphics[width=0.99\columnwidth, height=0.4\columnwidth]{imgs/most_unfair.pdf}
 \caption{Trustpilot ratings for the top 10 websites with the highest frequency of unfavorable financial terms per category, compared with a randomly sampled set of 40 websites.}
\label{fig:user_star}
\end{figure}

==> fig_tex/user_star_old.tex <==
\begin{figure*}[ht!]
\centering
\subfigure[Trustpilot ratings for websites with the top 10 highest frequency of unfavorable financial terms per category.]{
\label{fig:least-fairs-star}
    \includegraphics[width=0.25\textwidth, height=0.2\textwidth]{imgs/placeholder.png}
}
\subfigure[Trustpilot ratings for a randomly sampled set of 40 websites with no unfavorable financial terms.]{
\label{fig:least-unfair-star}
\includegraphics[width=0.25\textwidth, height=0.2\textwidth]{imgs/placeholder.png}
}
\subfigure[ScamAdvisor Trust Scores for websites with the top 10 highest frequency of unfavorable financial terms per category.]{
\label{fig:least-fairs-scam-score}
\includegraphics[width=0.25\textwidth, height=0.2\textwidth]{imgs/placeholder.png}
}

\caption{
Comparison of user ratings and trust scores for websites with and without unfavorable financial terms. 
}
\label{fig:user_star_old}
\end{figure*}

%
%
%

==> tables/classification_results_old.tex <==
\begin{table*}[!ht]
\centering
\begin{tabular}{llcccccc}
\toprule
\multirow{2}{*}{\textbf{Category}} & \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c}{\textbf{Simple Prompt}} & \multicolumn{3}{c}{\textbf{Malicious Taxonomy Prompt}} \\
\cmidrule{3-8}
& & \textbf{Precision} & \textbf{Recall} & \textbf{F1} & \textbf{Precision} & \textbf{Recall} & \textbf{F1} \\
\midrule
\multirow{4}{*}{\parbox{4cm}{Purchase and Billing Terms}} & GPT 3.5 & 0.23 & 0.78 & 0.36 & 0.26 & 0.97 & 0.41 \\
& GPT 4o & 0.29 & 0.88 & 0.43 & 0.48 & 0.94 & 0.64 \\
& Llama 3 & 0.25 & 0.84 & 0.38 & 0.34 & 0.94 & 0.50 \\
& Gemma & 0.26 & 0.71 & 0.38 & 0.27 & 1.00 & 0.42\\
\midrule
\multirow{4}{*}{\parbox{4cm}{Post-Purchase Terms}} 
& GPT 3.5 & 0.31 & 0.76 & 0.44 & 0.34 & 0.94 & 0.55 \\
& GPT 4o & 0.38 & 0.86 & 0.52 & 0.58 & 0.92 & 0.71\\
& Llama 3 & 0.33 & 0.82 & 0.47 & 0.41 & 0.82 & 0.54\\
& Gemma & 0.36 & 0.72 & 0.48 & 0.36 & 0.96 & 0.55 \\
\midrule
\multirow{4}{*}{\parbox{4cm}{Termination and Account Recovery Terms}} 
& GPT 3.5 & 0.13 & 0.75 & 0.22 & 0.14 & 0.88 & 0.24\\
& GPT 4o & 0.19 & 1.00 & 0.31 & 0.33 & 1.00 & 0.50\\
& Llama 3 & 0.15 & 0.88 & 0.25 & 0.17 & 0.75 & 0.28\\
& Gemma & 0.19 & 0.94 & 0.32 & 0.16 & 1.00 & 0.27 \\
\midrule
\multirow{4}{*}{\parbox{4cm}{Legal Terms}} 
& GPT 3.5 & 0.24 & 0.84 & 0.37 & 0.25 & 0.97 & 0.40\\
& GPT 4o & 0.31 & 1.00 & 0.47 & 0.40 & 0.88 & 0.50 \\
& Llama 3 & 0.25 & 0.87 & 0.39 & 0.28 & 0.71 & 0.40 \\
& Gemma & 0.33 & 0.97 & 0.49 & 0.27 & 1.00 & 0.43 \\
\midrule
\midrule
\multirow{4}{*}{\parbox{4cm}{All Unfavoravle Terms Combined}} & GPT 3.5 & 0.55 & 0.78 & 0.64 & 0.58 & 0.95 & 0.72 \\
& GPT 4o & 0.63 & 0.91 & 0.74 & 0.78 & 0.88 & 0.82 \\
& Llama 3 & 0.57 & 0.84 & 0.68 & 0.64  & 0.81  & 0.72\\
& Gemma & 0.62 & 0.81 & 0.70 & 0.60 & 0.98 & 0.74\\
\midrule
\multirow{4}{*}{Benign} 
& GPT 3.5 & 0.55 & 0.29 & 0.38 & 0.81 & 0.25 & 0.38\\
& GPT 4o & 0.81 & 0.40 & 0.54 & 0.84 & 0.73 & 0.78 \\
& Llama 3 & 0.64 & 0.30 & 0.41 & 0.71 & 0.50 & 0.59 \\
& Gemma & 0.68 & 0.45 & 0.54 & 0.94 & 0.27 & 0.42 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/per_category_analysis.tex <==
\begin{table}[!ht]
\centering
\footnotesize
\caption{Performance metrics per category for a selected group of configurations.}
\label{tab:per_cat}
\begin{tabular}{p{1.6cm} p{2.2cm} p{1.2cm} p{1.2cm} }
\toprule
\textbf{Category} & \textbf{Model} & \textbf{FPR (\%)} & \textbf{TPR (\%)} \\
\midrule
\multirow{2}{*}{\shortstack[l]{Purchase and\\Billing Terms}} 
& GPT-4o & 40.9 & 88.0 \\
& GPT-3.5-Turbo & 48.1 & 100.0 \\
& FT:GPT-3.5-Turbo & 0.0 & 84.6 \\
\midrule
\multirow{2}{*}{\shortstack[l]{Post-Purchase\\Terms}} 
& GPT-4o & 22.2 & 100.0 \\
& GPT-3.5-Turbo & 25.0 & 86.7 \\
& FT:GPT-3.5-Turbo & 0.0 & 100 \\

\midrule
\multirow{2}{*}{\shortstack[l]{Termination\\ and Account\\Recovery Terms}} 
& GPT-4o & 28.9 & 100.0 \\
& GPT-3.5-Turbo & 54.0 & 100.0  \\
& FT:GPT-3.5-Turbo & 14.8 & 93.3 \\

\midrule
\multirow{2}{*}{\shortstack[l]{Legal Terms}} 
& GPT-4o & 24.13 & 97.7 \\
& GPT-3.5-Turbo & 36.20 &  95.5  \\

& FT:GPT-3.5-Turbo  & 13.3 & 90.9 \\


\bottomrule
\end{tabular}

\end{table}


